EasyControl: Transfer ControlNet to Video Diffusion for Controllable Generation and Interpolation

Following the advancements in text-guided image generation technology exemplified by Stable Diffusion, video generation is gaining increased attention in the academic community. However, relying solely on text guidance for video generation has serious limitations, as videos contain much richer content than images, especially in terms of motion. This information can hardly be adequately described with plain text. Fortunately, in computer vision, various visual representations can serve as additional control signals to guide generation. With the help of these signals, video generation can be controlled in finer detail, allowing for greater flexibility for different applications. Integrating various controls, however, is nontrivial. In this paper, we propose a universal framework called EasyControl. By propagating and injecting condition features through condition adapters, our method enables users to control video generation with a single condition map. With our framework, various conditions including raw pixels, depth, HED, etc., can be integrated into different Unet-based pre-trained video diffusion models at a low practical cost. We conduct comprehensive experiments on public datasets, and both quantitative and qualitative results indicate that our method outperforms state-of-the-art methods. EasyControl significantly improves various evaluation metrics across multiple validation datasets compared to previous works. Specifically, for the sketch-to-video generation task, EasyControl achieves an improvement of 152.0 on FVD and 19.9 on IS, respectively, in UCF101 compared with VideoComposer. For fidelity, our model demonstrates powerful image retention ability, resulting in high FVD and IS in UCF101 and MSR-VTT compared to other image-to-video models.

==> sec/3_pre.tex <==
\section{Preliminary}

\textbf{Diffusion models (DMs)~\cite{2020DMs}} is a probabilistic generative model that learns the underlying data distribution through two steps: diffusion and denoising. Specifically, during the diffusion process, given an input data $\mathbf{z}$, the model gradually adds random noise $ \mathbf{z}_{t} = \alpha_{t}\mathbf{z} + \sigma_{t}\epsilon $, where $ \epsilon \in \mathcal{N}(\mathbf{0}, \mathbf{I}) $. The magnitudes of noise addition are controlled by $ \alpha_{t} $ and $ \sigma_{t} $ as the denoising steps $t$ progress. In the following denoising stage, the model takes the diffused sample $ \mathbf{z}_{t} $ as input and minimizes the mean squared error loss to learn a denoising function $ \epsilon_{\theta} $ as follows: 
%
\begin{equation}
    E_{\mathbf{z},\epsilon,t}=\left[ \lVert \epsilon_{\theta}(\mathbf{z}_{t}, t) - \epsilon \lVert \right]
\end{equation}


\noindent \textbf{Latent Diffusion Models (LDMs)~\cite{LDMs}} utilize the architecture of Variational Autoencoders (VAEs). Unlike Diffusion Models (DMs), LDMs can compress the input data into a latent variable $ \epsilon(\mathbf{z}) $ by encoder $ \epsilon $, and then perform denoising truncation by decoding $D(\mathbf{z}_{0})$ by the decoder $D$. LDMs significantly reduce the training and inference time as the diffusion and denoising are performed in the latent space rather than the data space. The objective of LDMs can be formulated as follows:
%
\begin{equation}
    E_{\mathbf{z},\epsilon,t}=\left[ \lVert \epsilon_{\theta}(\mathcal{E}(\mathbf{z}_{t}), t) - \epsilon \lVert \right]
\end{equation}


\noindent \textbf{Video Latent Diffusion Models (VLDMs)} build upon LDMs by incorporating a temporal module to capture the temporal continuity in video data. VLDMs typically add a temporal attention module to the U-Net architecture, enabling attention in the temporal dimension. Additionally, the 2d convolutions are modified to 3d convolutions to accommodate video data. Given the impressive capabilities of VLDMs in video generation, our proposed approach, dragVideo, follows the principles of VLDMs, which encodes video into latent variables $ \mathcal{E}(\mathbf{z}) $ and leverages U-Net to learn the spatio-temporal characteristics of the video data.



